PMGDA: A Preference-based Multiple Gradient Descent Algorithm

It is desirable in many multi-objective machine learning applications, such as multi-task learning with conflicting objectives and multi-objective reinforcement learning, to find a Pareto solution that can match a given preference of a decision maker. These problems are often large-scale with available gradient information but cannot be handled very well by the existing algorithms. To tackle this critical issue, this paper proposes a novel predict-and-correct framework for locating a Pareto solution that fits the preference of a decision maker. In the proposed framework, a constraint function is introduced in the search progress to align the solution with a user-specific preference, which can be optimized simultaneously with multiple objective functions. Experimental results show that our proposed method can efficiently find a particular Pareto solution under the demand of a decision maker for standard multiobjective benchmark, multi-task learning, and multi-objective reinforcement learning problems with more than thousands of decision variables. Code is available at: https://github.com/xzhang2523/pmgda. Our code is current provided in the pgmda.rar attached file and will be open-sourced after publication.}

==> latex/app_matrix.tex <==
\appendix

\paragraph{Using \texttt{cvxopt} to solve linear programming problem (\eqref{eqn:project:dual}) }
The total number of variables is $m+2$. 
A \texttt{cvxopt} problem can be written as follows,
\begin{equation}
    \begin{aligned}
    & \min_x c^T x \\ 
    & \st A x \leq b.    
    \end{aligned}
\end{equation}
Here $c$ is the objective vector,
\begin{equation}
    c = [\underbrace{0,\ldots, 0}_{m+1}, -1].
\end{equation}
Here $A$ and $b$ are the constraint matrix and vector, containing 4 parts.

% \begin{equation}
%     A = [-G\hat{G}, A_2, A_3, A_4]. 
% \end{equation}
\begin{equation}
    A = \left [
    \begin{array}{cccc}
       \hline
       -1 & \ldots & 0 & 0 \\
       \vdots & \ddots & \vdots & 0 \\
       0 & \ldots & 1 & 0 \\
       \hline
       1 & \ldots & 1 & 0 \\ 
       \hline
       1 & \ldots & 1 & 0 \\ 
    \end{array}
    \right ]
\end{equation}
and 
\begin{equation}
    b = [b_1, -1 \ldots -1, 1, -1]^T.
\end{equation}


==> latex/conclu.tex <==
	


==> latex/exp.tex <==


	
\subsection{Fairness Classification Problems}
	\label{sec_mtl}
    We study the performance of our method on three fairness classification tasks: Adult \cite{asuncion2007uci}, Compass \cite{angwin2016machine}, and Default \cite{yeh2009comparisons}. 
    \subsubsection{Settings}
    The first objective is the standard cross-entropy loss. The second objective is the differentiable Difference of the Equality of Opportunity (DEO) indicator \cite{padh2021addressing}, selecting "sex" as the sensible attribute. The adult/Compass/Default dataset has 34,188/4,319/21,000 samples in the training set and 9769/1235/6000 samples in the testing set. The experiment settings largely followed the work of COSMOS \cite{ruchte2021cosmos}. 
    
    The classification model is a three-layer fully-connected neural network activated by ReLU, with 6891 parameters in Adult, 2811 parameters in Compass, and 7011 parameters in Default. All results were implemented with the PyTorch library \cite{paszke2019pytorch}. The learning rate is set to $10^{-3}$, the optimizer is Adam, and the batch size is 128. The parameter $\sigma$ is set to 0.85. 	
    \begin{table*}[htbp]
        \centering
        \begin{tabular}{cl|rr|rr|rr|rr}
            \toprule
            & \multicolumn{1}{r|}{} & \multicolumn{4}{c|}{Training dataset}    & \multicolumn{4}{c}{Testing dataset} \\ 
            Task & Method &  KLE($10^{-3}$) $\downarrow$ & (std) & PBI ($10^{-2}$) $\downarrow$  & (std) & KLE ($10^{-3}$) $\downarrow$ & (std) & PBI ($10^{-2}$) $\downarrow$  & (std) \\ \midrule
            \multirow{3}[0]{*}{Adult}
          & PMGDA & \textbf{\underline{0.43}} & 0.11  & \textbf{8.75} & 0.14  & 
\textbf{\underline{2.52}} & 0.88  & \textbf{9.76} & 0.25 \\
          & EPO   & 2.68  & 0.07  & 10.17 & 0.01  & 4.15  & 1.19  & 11.21 & 0.37 \\
          & COSMOS & \textbf{0.11}   & 0.02  & 9.2   & 0.01  & \textbf{0.95}  & 0.44  & 10.17 & 0.05 \\
            \midrule
            \multirow{3}[0]{*}{Compass}
& PMGDA & 0.93  & 0.21  & 22.34 & 0.48  & \textbf{5.25} & 0.65  & 27.36 & 0.26 \\
          & EPO   & \textbf{0.09} & 0.02  & \textbf{19.65} & 0.15  & 5.87  & 1.13  & 26.99 & 0.8 \\
          & COSMOS & 7.4   & 0.22  & 22.99 & 0.1   & 12.19 & 0.94  & \textbf{26.89} & 0.54 \\
            \midrule
            \multirow{3}[0]{*}{Default}
          & PMGDA & 15.83 & 1.43  & \textbf{2.79} & 0.04  & \textbf{14.37} & 1.47  & \textbf{2.63} & 0.03 \\
          & EPO   & 23.14 & 0.74  & 2.86  & 0.04  & 38.37 & 2.2   & 3.18  & 0.03 \\
          & COSMOS & \textbf{9.46} & 1.97  & 2.99  & 0.17  & 18.84 & 1.24  & 3.32  & 0.06\\
            \bottomrule
        \end{tabular}%
        \caption{Our method is evaluated on three fairness classification tasks with ten given user preferences. All results are averaged over three random seeds. Our proposed method is able to search for solutions that best match user preferences. }
        \label{table_fair}%
    \end{table*}%
    \begin{figure*}[h] %%跨栏图为：figure*而单栏图为 figure
        \centering%52 44
        \subfigure[Training losses on Adult.]{\includegraphics[width=\hwidth \textwidth]{figure/experiment/adult/train_all_20.pdf}}
        \subfigure[Training losses on Compass.]{\includegraphics[width=\hwidth \textwidth]{figure/experiment/compass/train_all_20.pdf}}
        \subfigure[Training losses on Default.]{ \includegraphics[width=\hwidth \textwidth]{figure/experiment/default/train_all_20.pdf}}  \\
        \subfigure[Testing losses on Adult.]{\includegraphics[width=\hwidth \textwidth]{figure/experiment/adult/test_all_20.pdf}}
        \subfigure[Testing losses on Compass.]{\includegraphics[width=\hwidth \textwidth]{figure/experiment/compass/test_all_20.pdf}}
        \subfigure[Testing losses on Default.]{ \includegraphics[width=\hwidth \textwidth]{figure/experiment/default/test_all_20.pdf}}  \\
        \caption{Results on fairness classification tasks, Adult, Compass, and Default. COSMOS does not converge after the same iterations. Our solutions are closer to desired preferences in the difficult Adult and Default dataset. Behaviors on the easy Compass dataset by PMGDA, EPO, and COSMOS are similar. }
        \label{fig_mtl_all}
    \end{figure*}
    
    \begin{figure*}[h] %%跨栏图为：figure*而单栏图为 figure
        \centering%52 44
        \subfigure[Learning curve of PMGDA.]{ \includegraphics[width=\bwidth \textwidth]{figure/experiment/adult/traj_PMGDA_20_pbi.pdf}}
        \subfigure[Learning curve of EPO.]{ \includegraphics[width=\bwidth \textwidth]{figure/experiment/adult/traj_EPO_20_cel.pdf}}
        \subfigure[PBI indicator of PMGDA.]{ \includegraphics[width= \bwidth \textwidth]{figure/experiment/pbi/adult/pbi_PMGDA_train.pdf}}
		\subfigure[PBI indicator of EPO.]{ \includegraphics[width= \bwidth \textwidth]{figure/experiment/pbi/adult/pbi_EPO_train.pdf}}
        \caption{Comparison with PMGDA and EPO on training losses in the Adult dataset. Solutions generated by our method keep closer to given user preferences. }
        \label{fig_fair_compare}
    \end{figure*}
    \subsubsection{Results}
    The results of the experiments are shown in Table \ref{table_fair} and Figure \ref{fig_mtl_all}. We can observe that the solutions generated by the Linear scalarization (LS) method are only in a small region; for instance, on the Adult dataset, the LS method can only find solutions in the right-bottom corner. This phenomenon further emphasizes the necessity of finding exact solutions in order to get a set of diverse Pareto solutions. 
    
    The COSMOS method has the disadvantage of being difficult to choose the hyperparameter to balance the distance to the Pareto front and given preference. As Figure \ref{fig_mtl_all} shows, the solutions for the Adult and Default datasets have not converged to the Pareto front with $\mu=5.0$. As a result, the PBI indicator on Adult and Default datasets is large. On the Compass dataset, the generated solutions do not appear to fit user preferences very well, as evidenced by the fact that the KLE indicator of Compass is significantly larger than the KLE indicators of the other two methods.
    
    We illustrate the difference between our proposed method and the Exact Pareto Optimization (EPO) method on the Adult dataset in Figure \ref{fig_fair_compare}. Around half of the solutions generated by EPO fail to accurately match user preferences, while solutions generated by our approach remain close to the specified user preferences. This is further evidenced by Table \ref{table_fair}, which shows that the KLE and PBI indicators of our method are much lower than those of the EPO on the Adult and Default datasets. On the easiest Compass dataset, both KLE indicators of our method and EPO are relatively low.
    
    The searching mechanism of the EPO method is quite complex since it divides the $m$ objectives into three index sets $J,\overline{J}, J^*$ and addresses them differently, which can lead to linear programming problems with no feasible solutions. Despite its complexity, it is not yet clear how EPO can consistently generate exact Pareto solutions. We have adjusted various hyperparameters in order to generate solutions more aligned with user preferences. Despite these changes, the results remain largely similar to the results from the original implementations.
    \begin{figure*}[h] %%跨栏图为：figure*而单栏图为 figure
		\centering%52 44
		\subfigure[Objective 1 under pref {[0.17,0.83]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.17_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.29,0.71]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.29_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.40,0.60]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.40_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.52,0.48]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.52_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.63,0.37]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.63_seed_all_left.pdf}} 
		\\
		\subfigure[Objective 1 under pref {[0.17,0.83]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.17_seed_all_right.pdf}} 
		\subfigure[Objective 1 under pref {[0.29,0.71]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.29_seed_all_right.pdf}} 
		\subfigure[Objective 1 under pref {[0.40,0.60]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.40_seed_all_right.pdf}} 
		\subfigure[Objective 1 under pref {[0.52,0.48]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.52_seed_all_right.pdf}} 
		\subfigure[Objective 1 under pref {[0.63,0.37]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_traj_pref_0.63_seed_all_right.pdf}} 
		\caption{Learning curves of MO-HalfCheetah. Our method fits well with the red line, which is the best solution satisfying the exact requirement. }
		\label{fig_rl_hc}
    \end{figure*}
	
    \begin{figure*}[h] %%跨栏图为：figure*而单栏图为 figure
		\centering%52 44
		\subfigure[Objective 1 under pref {[0.17,0.83]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.17_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.34,0.66]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.34_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.51,0.49]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.51_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.67,0.33]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.67_seed_all_left.pdf}} 
		\subfigure[Objective 1 under pref {[0.84,0.16]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.84_seed_all_left.pdf}} 
		\\
		\subfigure[Objective 2 under pref {[0.17,0.83]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.17_seed_all_right.pdf}} 
		\subfigure[Objective 2 under pref {[0.34,0.66]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.34_seed_all_right.pdf}} 
		\subfigure[Objective 2 under pref {[0.51,0.49]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.51_seed_all_right.pdf}} 
		\subfigure[Objective 2 under pref {[0.67,0.33]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.67_seed_all_right.pdf}} 
		\subfigure[Objective 2 under pref {[0.84,0.16]}]{ \includegraphics[width=\dwidth \textwidth]{figure/experiment/mujoco/Ant_traj_pref_0.84_seed_all_right.pdf}} 
		\caption{Learning curves of MO-Ant. Our method fits well with the red line, which is the best solution satisfying the exact requirement. }
		\label{fig_rl_ant}
    \end{figure*}
	
	
    \subsection{Multi-objective Reinforcement Learning (MORL)}
    In this section, we study the performance of our method on two deep MORL tasks \cite{xu2020prediction}. MORL tasks are very difficult to train, and the gradients estimated by RL algorithms are usually noisy. This part illustrates that our method can scale well to complex practical tasks. The two tasks are:
    \begin{itemize}
		\item[-] MO-HalfCheetah. The first and second objectives are to maximize the forward velocity and energy efficiency. The dimension of observation and action space is 17 and 6.
		\item[-] MO-Ant. The first and second objectives are to maximize the x-axis and y-axis velocities. The dimension of observation and action space is 111 and 8.
    \end{itemize}
    
    We do not include the result of EPO for MORL since EPO is only designed for minimization problems with positive objectives. It is unclear how to extend EPO for multi-objective maximization problems. Our method can be easily extended for maximization problems by maximizing the inner product of descending directions and the policy gradients are the prediction step.
    \subsubsection{Settings}
    For MORL tasks, the cosine similarity term is very small ($\leq 1$) compared to the linear scalarization term. To encourage solution similarities, we set the control parameter of the cosine similarity term to a very large value (1000).  
    
    MO-HalfCheetah is trained for 3.28 million timesteps with control parameter $\sigma=0.1$. Compared with MO-HalfCheetah, MO-Ant has a much more complex structure. In order to speed up the convergence, we use linear scalarization to pretrain the model for 11.47 million time steps and set $\sigma=0.0$. 	
	\begin{table*}[htbp]
		\centering
		\begin{tabular}{cl|rr|rr|rr}
			\toprule
			&       & \multicolumn{1}{l}{PMGDA} & (std) & \multicolumn{1}{l}{LS} & (std)  & \multicolumn{1}{l}{COSMOS} & (std)  \\
			\midrule
			\multirow{2}[0]{*}{MO-HC} & KLE($10^{-3}$) $\downarrow$   & \textbf{0.42} & 0.1   & 47.49 & 19.25 & 21.56 & 1.79 \\
			& PBI ($10^3$) $\uparrow$    & 
    \textbf{2.58} & 0.04  & 1.2   & 0.41  & 1.74  & 0.12       \\
			\midrule
			\multirow{2}[0]{*}{MO-Ant} & KLE($10^{-3}$) $\downarrow$    & \textbf{4.05} & 0.93  & 55.99 & 7.93  & 30.92 & 6.08 \\
			& PBI ($10^3$) $\uparrow$    & \textbf{2.34} & 0.12  & 0.7   & 0.13  & 1.27  & 0.26 \\
			\bottomrule
		\end{tabular}%
		\caption{Results on Multi-objective reinforcement learning tasks. Our method can consistently search for high-quality Pareto solutions. The KLE of our method is closer to zero and the PBI indicator is higher than other methods.}
		\label{table_rl_all}%
	\end{table*}%
    Gradient vectors $\nabla L_1(\vth)$, $\nabla L_2(\vth)$ for all methods are estimated via the Proximal Policy Optimization (PPO) algorithm \cite{schulman2017proximal} and a critic network $V_\phi$ is trained to reduce the variance of the estimated gradients. Hyper-parameters of PPO follow the settings in \cite{xu2020prediction}.
    \subsubsection{Results}
    The results of the total reward learned by different methods are shown in Figure \ref{fig_rl_all} and Table \ref{table_rl_all}. And the learning curves on MO-HalfCheetah and MO-Ant are shown in Figure \ref{fig_rl_hc} and \ref{fig_rl_ant}. Figure \ref{fig_rl_all} and Table \ref{table_rl_all} clearly show that only our method can search for exact Pareto solutions. Our method generally produces solutions that fit well with the user preference vectors, while the other two methods often fail to fit user preference in most cases. As a result, our method achieves much lower KLE and higher PBI indicators on both problems. The KLE indicator of COSMOS is lower than LS, indicating that the cosine similarity term is helpful to search for exact solutions. 
    
    Figure \ref{fig_rl_hc} (a), (b), (f), and (g) show that the LS and COSMOS methods find duplicate Pareto solutions under preferences $[0.17,0.83]$ and $[0.29,0.71]$. This phenomenon further proves the necessity of finding an exact solution. Our method generates more diverse solutions when given a fixed number of preference vectors. 
    
    A red line in Figures \ref{fig_rl_hc} and \ref{fig_rl_ant} indicates the best exact Pareto solution. This solution has the highest projection value on a given preference vector and is able to satisfy the exact constraint with a small margin.  As can be seen from Figure \ref{fig_rl_hc} and \ref{fig_rl_ant}, the learning curve of our method is generally close to the red lines, indicating that the proposed searching mechanism is stable. 
    
    \begin{figure}
		\centering
		\subfigure[Results on MO-HC]{ \includegraphics[width=\cwidth \textwidth]{figure/experiment/mujoco/HalfCheetah_seed_All.pdf}}
		\subfigure[Results on MO-Ant]{ \includegraphics[width=\cwidth \textwidth]{figure/experiment/mujoco/Ant_seed_All.pdf}} 
		\caption{Results on multi-objective deep RL tasks. Our solutions can better fit given preference vectors than other methods. }
		\label{fig_rl_all}
    \end{figure}
    
    The number of parameters of different tasks is shown in Table \ref{table_param}.

    
    \begin{table}[]
        \begin{tabular}{llllll}
        \toprule
        Problem & Adult  & Compass & Default & HalfCheetah & Ant\\ 
        \#Params & 6891 & 2811 & 7011 & 10754 & 12034 \\
        \bottomrule
        \end{tabular}
        \caption{Number of model parameters.} \label{table_param}
    \end{table}

==> latex/introduction.tex <==




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}



% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}


% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}


\def\secref#1{section~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Secref#1{Section~\ref{#1}}

\def\tableref#1{table~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Tableref#1{Table~\ref{#1}}

\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.

\def\Secref#1{Section~\ref{#1}}

\def\Lemref#1{Lemma~\ref{#1}}
\def\Thref#1{Theorem~\ref{#1}}
\def\Propref#1{Proposition~\ref{#1}}

% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation (\ref{#1})}
% Reference to an equation, upper case
\def\Eqref#1{Equation (\ref{#1})}
\def\Probref#1{Problem (\ref{#1})}


% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}
\def\Tau{\mathcal{T}}

% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

\newtheorem{example}{Example}
\newtheorem{theorem}{Theorem}
\newtheorem{informaltheorem}[theorem]{(Informal) Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{property}{Property}
\newtheorem{definition}{Definition}
\newtheorem{lemma}{Lemma}
\newtheorem{fact}{Fact}
\newtheorem{corollary}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{remark}{Remark}

\newcommand{\norm}[1]{\left\lVert#1\right\rVert}
% \newcommand{\norm2}[1]{{\left\lVert#1\right\rVert}^2}
\newcommand{\abs}[1]{\left\lvert#1\right\rvert}

